A learning-based projection method for model order reduction of transport problems

The Kolmogorov $n$-width of the solution manifolds of transport-dominated problems can decay slowly. As a result, it can be challenging to design efficient and accurate reduced order models (ROMs) for such problems. To address this issue, we propose a new learning-based projection method to construct nonlinear adaptive ROMs for transport problems. The construction follows the offline-online decomposition. In the offline stage, we train a neural network to construct adaptive reduced basis dependent on time and model parameters. In the online stage, we project the solution to the learned reduced manifold. Inheriting the merits from both deep learning and the projection method, the proposed method is more efficient than the conventional linear projection-based methods, and may reduce the generalization error of a solely learning-based ROM. Unlike some learning-based projection methods, the proposed method does not need to take derivatives of the neural network in the online stage.

==> removed_1d_riemann_example.tex <==
%%%%%%%%%%%%%%%
\subsubsection{Future prediction for a Riemann problem \label{sec:burgers_prediction}}
We consider the computational domain $[0,6]$ and the initial condition 
\begin{align}
    u(x,0) = \begin{cases}
             1.,\quad %\text{if}\;
             x\in[2,3],\\
             0.,\quad\text{otherwise.}
             \end{cases}
\end{align}
The solution of this problem has  a rarefaction fan and a moving shock simultaneously. We use a uniform mesh with $\Dx=0.02$ and the time step size \mw{is taken to be} $\Dt=0.25\Dx$. The training set is the full order numerical solution  for $t\in[0,2]$. We will predict the solution at future time from $t=2$ to $t=4$, and compare our method with the POD method and the pure learning method.
The neural network is trained with $500$ epochs.

In Figure \ref{fig:burgers_prediction_error_vs_order}, \mw{we present the largest relative prediction error from $t=2$ to $t=4$ versus the reduced order $r$}. As the number of basis grows, the relative errors of the POD method and the LP method decay, while the relative error of the learning method may not. This is likely due to over-fitting.  
For a given reduced order $r$, the LP method \mw{constantly} results in the smallest relative error. For example, with $r=30$, the LP method achieves less than $0.6\%$ relative error, while the error of the POD method with the same number of basis is more than $40\%$ and \pzc{the error of the pure learning based method is \mw{over} $30\%$}. The results thus far show that the online projection step effectively reduces the generalization error \mw{produced in} the  learning \mw{step}. In addition, with the learned adaptive basis, the LP method significantly outperforms the conventional POD method. 

In Figure \ref{fig:burgers_prediction_solution}, we present the predicted  solutions at $t=4$ with $r=10, 20, 30$.  
We find that the solutions by the LP method match the full order solution the best,  especially in capturing the shock location.  In Figure \ref{fig:burgers_prediction_error_history}, the time evolution of the $L_2$ error for different methods is presented under the $\log$-scale. Though initially the POD method displays the smallest error with $20$ basis functions, \mw{this} error grows very fast. For $t\geq 2.25$, the LP method always achieves the smallest error. When $30$ reduced basis functions are used, the error of the LP method grows slowly. When predicting solutions with shock features by ROMs, it is important to  control numerical oscillations effectively. When $r=10$, 
some oscillations are observed in the solutions by the LP method. These  oscillations become invisible once more basis functions are used. It is possible to  apply the $L_1$ minimization framework \cite{abgrall2018model} online to better control the numerical oscillations.


%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\centering
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{picture/burgers/relative_error_vs_order.png}
  \caption{Comparison between pure learning, POD and the LP method}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{picture/burgers/relative_error_vs_order_zoom_in.png}
    \caption{Zoomed-in picture}
\end{subfigure}
\caption{x axis: Reduced order $r$. y axis: The largest relative prediction error \mw{among $t\in[2,4]$} 
for the Burgers equation (Riemann problem) in Section \ref{sec:burgers_prediction}.\label{fig:burgers_prediction_error_vs_order}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\centering
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{picture/burgers/solution10.png}
  \caption{10 basis functions}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{picture/burgers/solution20.png}
  \caption{20 basis functions}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{picture/burgers/solution30.png}
  \caption{30 basis functions}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{Predicted solutions of the Burgers equation (Riemann problem) in Section \ref{sec:burgers_prediction} 
at $t=4.0$.\label{fig:burgers_prediction_solution}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
\centering
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{picture/burgers/error_evolution10.png}
  \caption{$10$ basis functions}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{picture/burgers/error_evolution20.png}
  \caption{$20$ basis functions}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\textwidth]{picture/burgers/error_evolution30.png}
  \caption{$30$ basis functions}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{The time evolution of the prediction error for \mw{$t\in[2,4]$ of} the Burgers equation (Riemann problem) in Section \ref{sec:burgers_prediction}.\label{fig:burgers_prediction_error_history}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%
